Charm physics at BESIII

The study of mesons and baryons which contain at least one charm quark is referred to as open charm physics. It offers the possibility to study up-type quark transitions. Since the $c$ quark can not be treated in any mass limit, theoretical predictions are difficult and experimental input is crucial. BESIII collected large data samples of $e^{+}e^{-}$ collisions at several charm thresholds. The at-threshold decay topology offers special opportunities to study open charm decays. We present a selection of recent BESIII results. Branching fractions and the $D_{s}^{+}$ decay constant are measured using the leptonic decays to $\mu^{+}\nu$ and $\tau^{+}\nu$. From a data sample of $0.482 fb^{-1}$ collected at the $D_{s}^{+}D_{s}^{-}$ threshold we measure $f_{Ds}=(241 \pm 16.3(stat.) \pm 6.6(sys.)) MeV$. BESIII recently found preliminary evidence of the decay $D_{s}^{+}\rightarrow\tau^{+}\nu$ and with a significance larger than $4 \sigma$ using $2.81 fb^{-1}$ of data at the $D^0\overline{D^0}$ threshold. Using the same data sample the decay $D^0\rightarrow K^0_{S/L} \pi^0(\pi^0)$ is analysed. The branching fractions are measured and using the $CP$ eigenstates $K_{S/L}^0\pi^0$ the $D^0$ mixing parameter $y_{CP} = (0.98 \pm 2.43)\%$ is measured.

==> alias.tex <==
\RequirePackage{xspace}


\newcommand{\ie}{i.\,e.\xspace}
\newcommand{\Ie}{I.\,e.\xspace}
\newcommand{\eg}{e.\,g.\xspace}
\newcommand{\Eg}{E.\,g.\xspace} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% DEPRECATED %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\GeV}{\si{\giga\electronvolt}\xspace}
\newcommand{\MeV}{\si{\mega\electronvolt}\xspace}
\newcommand{\KeV}{\si{\kilo\electronvolt}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% EXPERIMENTS %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\textbf\sl B}\hspace{-0.1em}{\LARGE\textbf\sl A}\hspace{-0.03em}{\huge\textbf\sl B}\hspace{-0.1em}{\LARGE\textbf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}

\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}\xspace}
\def\pep2{PEP-II}
\newcommand{\panda}{PANDA\xspace}
\newcommand{\bes}{BESIII\xspace}
\newcommand{\besSc}{\fontfamily{ppl}\selectfont\textsc{Besiii}\normalfont\xspace}
\newcommand{\lhcb}{LHCb\xspace}
\newcommand{\cleo}{\textsc{Cleo}\xspace}
\newcommand{\cleoc}{\cleo-c\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% SOME DEFS %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\particle}[1]{{\ensuremath{\mathrm #1}}\xspace}
%\newcommand{\BAR}[1]{\overline{#1}}
\newcommand{\BAR}[1]{\kern 0.2em\overline{\kern -0.2em #1}{}\xspace}
%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

%overline for normal text
\makeatletter
\newcommand*{\textover}[1]{\ensuremath{\overline{\hbox{#1}}\m@th}}
\makeatother

%\newcommand{\sgn}{\mathop{\mathrm{sgn}}} %sign operator; requires amsmath
\DeclareMathOperator{\sgn}{sgn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\numu        {\ensuremath{\nu_\mu}\xspace}
\def\numub       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\def\pion   {\ensuremath{\pi}\xspace}
\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\mathrm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}
\def\etapr {\ensuremath{\eta^\prime}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\KKbar {\ensuremath{\kaon\Kbar}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
%\def\KK    {\ensuremath{\KpKm}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KSL    {\ensuremath{K^0_{\scriptscriptstyle S/L}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\DD      {\ensuremath{D\Dbar}\xspace} 
\def\DDbar   {\DD\xspace}
\def\D       {\ensuremath{D}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\kern 0.2em\overline{\kern -0.2em D}\rule{0pt}{1.5ex}^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Dsp      {\ensuremath{D^+_s}\xspace}
\def\Dsm      {\ensuremath{D^-_s}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsd      {\ensuremath{D_{s(d)}}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}
\def\DsDsb   {\ensuremath{\Dsp{\kern -0.16em \Dsm}}\xspace}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace}
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace}
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}

% added by GHM on March 25, 2003 -- from Andrei Gritsan
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% QUARKONIA %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\psipp 	  {\psiprpr}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\p      	 {\proton\xspace}
\def\pbar      	 {\antiproton\xspace}
\def\ppbar       {\proton\antiproton\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}
\def\n 			 {\neutron\xspace}
\def\nbar 		 {\antineutron\xspace}
\def\nnbar 		 {\neutron\antineutron\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\mathcal B}}\xspace}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace}

\def\BtoDK      {\ensuremath{B \to DK}\xspace}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace}

\def\Btoetah    {\ensuremath{B \to \eta h}\xspace}
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace}

\def\btosgam    {\ensuremath{b \to s \g}\xspace}
\def\btodgam    {\ensuremath{b \to d \g}\xspace}
\def\btosll     {\ensuremath{b \to s \ellell}\xspace}
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace}
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace}
\def\btosglue   {\ensuremath{b \to s g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{\ensuremath{p}}\xspace}
\def\pt         {\mbox{\ensuremath{p_T}}\xspace}
\def\mes        {\mbox{\ensuremath{m_{\mathrm ES}}}\xspace}
\def\mec        {\mbox{\ensuremath{m_{\mathrm EC}}}\xspace}
\def\DeltaE     {\mbox{\ensuremath{\Delta E}}\xspace}
\def\qsq        {\ensuremath{q^2}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{\ensuremath{\phi}}\xspace}
\def\mtheta     {\mbox{\ensuremath{\theta}}\xspace}
\def\ctheta     {\mbox{\ensuremath{\cos\theta}}\xspace}
\def\cosTheta 	{\ensuremath{\cos(\Theta)}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   UNITS   %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareSIUnit\c{c}
\DeclareSIUnit\cSq{\c^2}
\DeclareSIUnit\eV{\tera\electronvolt}
\DeclareSIUnit\eVc{\electronvolt/\c}
\DeclareSIUnit\eVcSq{\electronvolt/\cSq}
\DeclareSIUnit\KeV{\kilo\electronvolt}
\DeclareSIUnit\MeV{\mega\electronvolt}
\DeclareSIUnit\GeV{\giga\electronvolt}
\DeclareSIUnit\TeV{\tera\electronvolt}
\DeclareSIUnit\invfb{\femto\barn\tothe{-1}}
\DeclareSIUnit\invpb{\pico\barn\tothe{-1}}
\DeclareSIUnit\timesten{\ensuremath{\times}10}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Some more (from Helen)
%\def\O{{\ensuremath{\mathcal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\mathcal O}}\xspace}
\def\L{{\ensuremath{\mathcal L}}\xspace}
\def\mathcalL{{\ensuremath{\mathcal L}}\xspace}
%\def\S{{\ensuremath{\mathcal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\mathcalS{{\ensuremath{\mathcal S}}\xspace}
\def\mathcalA{{\ensuremath{\mathcal A}}\xspace}
\def\mathcalD{{\ensuremath{\mathcal D}}\xspace}
\def\mathcalR{{\ensuremath{\mathcal R}}\xspace}

\def\jmathBar{{\ensuremath{\overline{\jmath}}}\xspace}
\def\imathBar{{\ensuremath{\overline{\jmath}}}\xspace}


\def\sx    {\ensuremath{\sigma_x}\xspace}     
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}

\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

% Data processing
\def\kbytes     {\ensuremath{{\mathrm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\mathrm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\mathrm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\mathrm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\mathrm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\mathrm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\mathrm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\mathrm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\mathrm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\mathrm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\mathrm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\mathrm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\mathrm \,Tbytes/yr}}\xspace}

% QCD parameters
\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters
\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}


% CKM, CP violation
\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
\def\CPV                {\ensuremath{C\!P\!V}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!
\def\C       {\ensuremath{C}\xspace}
\def\P       {\ensuremath{P}\xspace}
\def\G       {\ensuremath{P}\xspace}
\def\T       {\ensuremath{T}\xspace}
\def\JPC       {\ensuremath{J^{\P\C}}\xspace}
\def\JP       {\ensuremath{J^{\P}}\xspace}
\def\IG       {\ensuremath{I^{\G}}\xspace}

\def\epstag  {\ensuremath{\varepsilon_{\mathrm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\mathcal D}\xspace}
\def\deltaz{\ensuremath{{\mathrm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\mathrm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\mathrm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}
\newcommand{\qcd}{\ensuremath{\mathrm{QCD}}\xspace}
\newcommand{\QED}{\ensuremath{\mathrm{QED}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
%\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
%\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
%\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
%\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
%\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Meth.\xspace}
% update the following based on input from John Ripka, Asst. Editor at PRL, August 2006
\newcommand{\nimBaseA}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ A\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ B\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ C\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ D\xspace}
\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ E\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\textbf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\textbf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\textbf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\textbf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\textbf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\textbf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\textbf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\textbf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\textbf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\textbf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\textbf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\textbf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\textbf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\textbf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\textbf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\textbf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\textbf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\textbf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\textbf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\textbf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\textbf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\textbf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\textbf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\textbf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\textbf A{\textbf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\textbf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\textbf #1}}}
%\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\textbf G{\textbf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\textbf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\textbf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\textbf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\textbf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\textbf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instrum.\ and Methods~{\textbf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\textbf #1}}
\newcommand{\nimaa}       [1]  {\nimBaseE~{\textbf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instrum.\ Methods~{\textbf A{\textbf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseA~{\textbf #1}}
\newcommand{\nimb}      [1]  {\nimBaseB~{\textbf #1}}
\newcommand{\nimc}      [1]  {\nimBaseC~{\textbf #1}}
\newcommand{\nimd}      [1]  {\nimBaseD~{\textbf #1}}
\newcommand{\nime}      [1]  {\nimBaseE~{\textbf #1}}
% add commands for NIM articles from earlier periods
% for NIM articles from 1981-1983
\newcommand{\oldnim}    [1]  {Nucl.\ Instrum.\ Methods Phys.\ Res.~{\textbf #1}}
% for NIM articles prior to 1981
\newcommand{\oldernim}  [1]  {Nucl.\ Instrum.\ Methods~{\textbf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\textbf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\textbf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\textbf B{\textbf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\textbf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\textbf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\textbf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\textbf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\textbf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\textbf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\textbf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\textbf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\textbf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\textbf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\textbf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\textbf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\textbf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\textbf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\textbf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\textbf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\textbf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\textbf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\textbf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\textbf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\textbf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\textbf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\textbf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\textbf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\textbf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\textbf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\textbf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\textbf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\textbf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\textbf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\textbf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\textbf #1}}}
\newcommand{\sci}       [1]  {{Science~{\textbf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\textbf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\textbf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\textbf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\textbf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\textbf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\textbf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\textbf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\textbf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\textbf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\textbf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sftName}[1]{\mbox{\textsc{#1}}\xspace} %
\def\aslund     {\sftName{Aslund}}
\def\bbsim      {\sftName{BBsim}}
\def\beast      {\sftName{Beast}}
\def\beget      {\sftName{Beget}}
\def\Bta        {\sftName{Beta}}
\def\betakfit   {\sftName{BetaKfit}}
\def\cornelius  {\sftName{Cornelius}}
\def\evtgen     {\sftName{EvtGen}}
\def\euclid     {\sftName{Euclid}}
\def\fitver     {\sftName{FitVer}}
\def\fluka      {\sftName{Fluka}}
\def\fortran    {\sftName{Fortran}}
\def\gcalor     {\sftName{GCalor}}
\def\geant      {\sftName{GEANT}}
\def\gheisha    {\sftName{Gheisha}}
\def\hemicosm   {\sftName{HemiCosm}}
\def\hepevt     {\sftName{HepEvt}}
\def\jetset74   {\sftName{Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\sftName{KoralB}}
\def\minuit     {\sftName{Minuit}}
\def\objegs     {\sftName{Objegs}}
\def\paw        {\sftName{Paw}}
\def\Root       {\sftName{Root}}
\def\squaw      {\sftName{Squaw}}
\def\stdhep     {\sftName{StdHep}}
\def\trackerr   {\sftName{TrackErr}}
\def\turtle     {\sftName{Decay~Turtle}}
\providecommand{\mLyX}{L\kern-.1667em\lower.25em\hbox{Y}\kern-.125emX\@}
\def\COMPWA {\sftName{ComPWA}}
\def\MINUIT {\sftName{Minuit}}
\def\MIGRAD {\sftName{Migrad}}
\def\MINOS 	{\sftName{Minos}}
\def\HESSE  {\sftName{Hesse}}
\def\Minuit {\sftName{Minuit}}
\def\Migrad {\sftName{Migrad}}
\def\Minos  {\sftName{Minos}}
\def\Hesse  {\sftName{Hesse}}
\def\BOSS   {\sftName{BOSS}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own aliases
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\DKsKK}{\ensuremath{\Dz\to\KsKK}\xspace}
\newcommand{\KsKK}{\ensuremath{\KS\KpKm}\xspace}
\newcommand{\Kppim}{\ensuremath{\Kp\kern -0.16em \pim}\xspace}
\newcommand{\pipiKK}{\ensuremath{\pipi\kern -0.16em\KpKm}\xspace}
\newcommand{\dtagZero}{\ensuremath{K^-\pi^+}\xspace}
\newcommand{\dtagOne}{\ensuremath{K^-\pi^+\pi^0}\xspace}
\newcommand{\dtagThree}{\ensuremath{K^-\pi^+\pi^-\pi^+}\xspace}
\newcommand{\bkgOne}{\ensuremath{\text{Bkg}_{\text{KS}}}\xspace}
\newcommand{\bkgTwo}{\ensuremath{\text{Bkg}_{\text{nonKS}}}\xspace}
\newcommand{\phiPiPi}{\ensuremath{\Dz\to(KK)_{\phi}(\pi\pi)_\rho}\xspace}

\newcommand{\Amp}{\ensuremath{{\mathcal M}}\xspace}
\newcommand{\lumi}{\ensuremath{{\mathcal L}}\xspace}
\newcommand{\FitPar}{\ensuremath{\boldsymbol\beta}\xspace}
\newcommand{\DPvar}{\ensuremath{\boldsymbol\xi}\xspace}
\newcommand{\mBC}{\ensuremath{m_{BC}}\xspace}
\newcommand{\mKS}{\ensuremath{m_{KS}}\xspace}
\newcommand{\mKK}{\ensuremath{m_{KK}}\xspace}
\newcommand{\helKK}{\ensuremath{\cos\theta_{KK}}\xspace}
\newcommand{\mKSKplus}{\ensuremath{m_{K^0K^+}}\xspace}
\newcommand{\mKSKminus}{\ensuremath{m_{K^0K^-}}\xspace}
\newcommand{\mKKsq}{\ensuremath{\mKK^{2}}\xspace}
\newcommand{\mKSKplusSq}{\ensuremath{\mKSKplus^{2}}\xspace}
\newcommand{\mKSKminusSq}{\ensuremath{\mKSKminus^{2}}\xspace}
\newcommand{\helicityTheta}{\ensuremath{\Theta_{KK}}\xspace}
\newcommand{\FLATTE}{Flatt\'{e}\xspace}

\newcommand{\pull}{\ensuremath{{\mathcal P}}\xspace}
\newcommand{\pValue}{\ensuremath{{\mathcal P}}\xspace}
\newcommand{\prob}{\ensuremath{{\mathcal P}}\xspace}
\newcommand{\likelih}{\ensuremath{{\mathcal L}}\xspace}

